Price equilibria with positive margins in loyal-strategic markets with discrete prices

In competitive supply chains (SCs), pricing decisions are crucial, as they directly impact market share and profitability. Traditional SC models often assume continuous pricing for mathematical convenience, overlooking the practical reality of discrete price increments driven by currency constraints. Additionally, customer behavior, influenced by loyalty and strategic considerations, plays a significant role in purchasing decisions. To address these gaps, this study examines a SC model involving one supplier and two manufacturers, incorporating realistic factors such as customer demand segmentation and discrete price setting. Our analysis shows that the Nash equilibria (NE) among manufacturers are not unique, we then discuss the focal equilibrium. Our analysis also reveals that low denomination factors can lead to instability as the corresponding game does not have NE. Numerical simulations demonstrate that even small changes in price increments significantly affect the competitive dynamics and market share distribution.

==> dec.tex <==
\begin{Declaration}
\noindent
I declare that this written submission represents my ideas in my own words and where others' ideas or words have been included, I have adequately cited and referenced the original sources. I declare that I have properly and accurately acknowledged all sources used in the production of this report. I also declare that I have adhered to all principles of academic honesty and integrity and have not misrepresented or fabricated or falsified any idea/data/fact/source in my submission. I understand that any violation of the above will be a cause for disciplinary action by the Institute and can also evoke penal action from the sources which have thus not been properly cited or from whom proper permission has not been taken when needed.

\DecSign[\today]

\end{Declaration}
%========================================================================

















==> pub.tex <==
%%%
\listofpublications


\noindent Put your publications from the thesis here. The packages \texttt{multibib} or \texttt{bibtopic} or \texttt{biblatex} or enumerate environment or thebibliography environment etc. can be used to handle multiple different bibliographies in the document.








%%======================================================================
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../mainrep"
%%% End: 








